DELTACON: A Principled Massive-Graph Similarity Function

How much did a network change since yesterday? How different is the wiring between Bob's brain (a left-handed male) and Alice's brain (a right-handed female)? Graph similarity with known node correspondence, i.e. the detection of changes in the connectivity of graphs, arises in numerous settings. In this work, we formally state the axioms and desired properties of the graph similarity functions, and evaluate when state-of-the-art methods fail to detect crucial connectivity changes in graphs. We propose DeltaCon, a principled, intuitive, and scalable algorithm that assesses the similarity between two graphs on the same nodes (e.g. employees of a company, customers of a mobile carrier). Experiments on various synthetic and real graphs showcase the advantages of our method over existing similarity measures. Finally, we employ DeltaCon to real applications: (a) we classify people to groups of high and low creativity based on their brain connectivity graphs, and (b) do temporal anomaly detection in the who-emails-whom Enron graph.

==> 420real_percent.tex <==
\addtolength{\subfigcapskip}{0.2cm}
\begin{figure}[tbh!]
\centering
         \vspace{0.3cm}
          %\subfigure[Circle graphs (C) with 100 nodes]{\label{fig:circles2p}\includegraphics[width=0.33\textwidth]{FIG/2percent_circles100.pdf}}
	%\subfigure[Path graphs (P) with 100 nodes]{\label{fig:paths2p}\includegraphics[width=0.33\textwidth]{FIG/2percent_chains100.pdf}}
	%\subfigure[{\bf \small{100-node clique (K) and star graphs (S) compared against derived graphs with fewer edges: \method is robust to the number of groups.}}]{\label{fig:syntheticP}\includegraphics[width=\columnwidth, trim=2cm 1cm 2cm 2cm]{FIG/2percent_robust_cliques_stars100.pdf}} \vspace{0.5cm}\\
	\subfigure[{\bf \small{Quality of \methodSlow and \method. Political Blogs: similarity scores between the original network and the derived networks with $p\%=\{2\%, 5\%, \ldots, 70\%, 80\%\}$ reverted edges. Note that (a) the distance grows with the corruption level, and (b) \method is accurate even for a small number of groups.}}]{\label{fig:polblogsP}\includegraphics[width=\columnwidth, trim=2cm 1cm 2cm 2cm]{FIG/polblogs_robust.pdf}}
    \caption{ \method's performance on real datasets.
}
    \label{fig:percent}
\end{figure}

%In the previous paragraphs, 
We saw that \methodSlow satisfies all the desired properties, %on synthetic and real graphs, 
while its runtime is not
an issue for graphs with up to a few millions of nodes. %Although our naive method, \methodSlow, is not scalable to billion-node graphs, \method is applicable
However, billion-node graphs call for \method, which is scalable both in theory and practice (lemma \ref{lem:complexity}, section \ref{subsect:scalability}). Here we answer two questions: 
\begin{itemize}%\addtolength{\itemsep}{-.62\baselineskip} 
\item How do the similarity scores of \method and \methodSlow compare?%, and more
%importantly, do the methods give the same ordering of similarities between pairs of graphs?
%is the order of the similarity scores found with \methodSlow maintained when using \method?  
\item How much do the \method similarity scores vary as we change the number of node groups?
\end{itemize}

\mypar{Datasets}
We use the 100-node synthetic graphs (cliques, circles, paths and stars) and their derived graphs with 1, 3 and 10 fewer edges.
Moreover, we create corrupted versions of the Political Blogs dataset; corruption of $p\%$ means that from all the possible edges between $n$ nodes,
$p\%$ of the edges are reverted (removed if existent, added if non-existent). In our experiments $p\%$ varies from $2\%$ to $80\%$, and the corruption is incremental
from smaller to bigger levels of corruption.
% = \{2\%, 20\%, 40\%, 60\%, 80\%\}$, where bigger
%percentage of corruption is additional to smaller percentages.
\reminder{Is this clear??? --> the corruption of edges is done incrementally from the smaller percentage of corruption to the bigger}
%For the synthetic graphs, we compute the similarity scores between the original graph of a specific type and the resulting graphs with 
%1, 2, 3 and 10 fewer edges. On the other hand, for the Political Blogs dataset we created 9 graphs which had 2\%, 10\%, 20\%, 30\%, 40\%,
%50\%, 60\%, 70\% and 80\% of the edges corrupted respectively. By corruption of x\% we mean that from all the possible edges between $n$ nodes,
%we change x\% of the edges in the following way: if an edge exists in the graph, we remove it; otherwise we add it. The smaller sets of changed
%edges are included in the bigger ones, i.e. the graph with 10\% corrupted edges has 8\% more corrupted edges than the graph with 2\% changed
%edges.

%\begin{figure}[tbh!]
%	\includegraphics[width=\columnwidth, trim=2cm 1cm 2cm 2cm]{FIG/2percent_polblogs.pdf}
%    \caption{
%    [Real Graphs] Robustness of \method's similarity scores to the number of node groups. Similarity scores are computed between the original political blogs network and the derived networks with p\% reverted edges.}
%    \label{fig:polblogsP}
%\end{figure}


\mypar{Analysis} For every pair of graphs, we compute the similarity score of \method by varying the %fraction of initialized nodes to $p\%$ = {1\%, 2\%, 5\%, 10\%, 15\%, 20\%, 25\%, 30\%}. 
number of groups from $g=10$ to $n$ (when $g=n$, \method is equivalent to \methodSlow).
For each number of groups, we run \method 10 times and, in the plots, we report the average similarity score,
as well as the standard deviation (the latter is tiny and not visible in the plots). %This is done, because \method randomly picks the nodes that are initialized, and so the similarity scores
%are not exactly the same in every run of \method.
%
%Based on figures \ref{fig:syntheticP}-\ref{fig:polblogsP} we observe the following:

\begin{observation}
In our experiments, \methodSlow and \method agree on the ordering of pairwise graph similarities.
\end{observation}
In Fig.~\ref{fig:polblogsP} the lines do not cross and appear to be parallel to the line $y=x$, which corresponds to identical scores for the two methods. In Fig.~\ref{fig:syntheticP} and \ref{fig:polblogsP}, we observe that more corruption in the derived graphs leads consistently to lower similarity to the original graph.

\begin{observation}
The similarity scores of \method are robust to the number of groups, $g$.
\end{observation}
Obviously the more groups \method uses, the closer are the similarity scores to the ideal similarity scores, i.e. scores of \methodSlow. 
%As the number of groups increases, \method's similarity scores go arbitrarily close to \methodSlow's scores. 
For instance, in Fig. \ref{fig:polblogsP}, when the blogs are grouped in pairs 
resulting in almost 750 groups, the similarity scores between the original network and the derived networks (with any level of corruption) are almost identical to the scores of \methodSlow.
However, even with few groups, the approximation of \methodSlow is very good.
%Only slight increase is observed as \method becomes more coarse and partitions the nodes in few groups. As the number of groups increases, \method's similarity
%scores go arbitrarily close to \methodSlow's scores. However, the runtime of the method increases with the number of groups, and thus the two conflicting facts
%need to be conciliated.
%That is, the similarity scores of \method diverge more from the scores of \methodSlow and, also, expose higher variability as the number of groups decrease.
The plots for the path and cycle graphs are on the same lines and are omitted due to space limitations.


\reminder{
\begin{observation}
The fewer nodes are used as seeds (or the more groups, $g$,  we partition the nodes), the bigger runtime is required, since the complexity of the algorithm is $O(g|\nodeSet| + |\edgeSet|)$. 
\end{observation}
}

\mypar{Remark} Not only the accuracy, but also the runtime increases with the number of groups; so, the speed and accuracy trade-offs need to be conciliated. Experimentally, it seems that a good compromise is achieved even for $g$ smaller than 100.
%Given that the runtime of the method increases with the number of groups, and thus the need for speed and accuracy need to be conciliated.
%Since the variability of the results is more significant and the runtime increases when the fraction of initialized nodes increases,  it seems that
%a fraction of nodes $p=10\%-15\%$ consists a good compromise between the small runtime and the distance from \methodSlow's similarity scores. 

%\paragraph{Observations}
%First, in Fig. \ref{fig:cliques2p}-\ref{fig:polblogs2p} we see that the removal/change of more edges leads to smaller similarity to the original
%graphs. In the majority of cases, we see that the similarity scores increase as the fraction of the initialized nodes increases, and their relative
%differences are maintained. Although there are oscillations in a few cases, we observe that the similarity score is always monotonic on the number of changed edges. 
%It is obvious that the percentage of initialized nodes affects the runtime of \method; the fewer nodes we initialize, the more times is \fabp run resulting
%in increase of \method's execution time. Therefore, it is clear that we want to find the ``best'' choice of $p$ that yields intuitive similarity scores, and
%at the same time keeps the runtime small. Since the variability of the results increases when the fraction of initialized nodes is bigger, it seems that
%any fraction of nodes up to 10\%-15\% satisfies our intuitivess and runtime requirements.
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{FIG/2percent_barbel.pdf}
%\label{fig:scalability}
%\caption{\method scales well for graphs with millions of edges.}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{FIG/2percent_cliques100.pdf}
%\caption{Similarity scores of \method on Clique graphs (K) with 100 nodes for different fraction of initialized nodes.}
%\label{fig:cliques2p}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{FIG/2percent_circles100.pdf}
%\caption{Similarity scores of \method on Circle graphs (C) with 100 nodes for different fraction of initialized nodes.}
%\label{fig:circles2p}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{FIG/2percent_chains100.pdf}
%\caption{Similarity scores of \method on Path graphs (P) with 100 nodes for different fraction of initialized nodes.}
%\label{fig:paths2p}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{FIG/2percent_stars100.pdf}
%\caption{Similarity scores of \method on Star graphs (S) with 100 nodes for different fraction of initialized nodes.}
%\label{fig:stars2p}
%\end{figure}
%
%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{FIG/2percent_polblogs.pdf}
%\caption{Similarity scores of \method on Political Blogs with 100 nodes for different fraction of initialized nodes.}
%\label{fig:polblogs2p}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{FIG/2percent_synthGraphs5.pdf}
%\label{fig:scalability}
%\caption{\method scales well for graphs with millions of edges.}
%\end{figure}

==> graph_similarity.tex <==
- features extraction
- frequent subgraph 
